NISP: Pruning Networks using Neuron Importance Score Propagation

To reduce the significant redundancy in deep Convolutional Neural Networks (CNNs), most existing methods prune neurons by only considering statistics of an individual layer or two consecutive layers (e.g., prune one layer to minimize the reconstruction error of the next layer), ignoring the effect of error propagation in deep networks. In contrast, we argue that it is essential to prune neurons in the entire neuron network jointly based on a unified goal: minimizing the reconstruction error of important responses in the "final response layer" (FRL), which is the second-to-last layer before classification, for a pruned network to retrain its predictive power. Specifically, we apply feature ranking techniques to measure the importance of each neuron in the FRL, and formulate network pruning as a binary integer optimization problem and derive a closed-form solution to it for pruning neurons in earlier layers. Based on our theoretical analysis, we propose the Neuron Importance Score Propagation (NISP) algorithm to propagate the importance scores of final responses to every neuron in the network. The CNN is pruned by removing neurons with least importance, and then fine-tuned to retain its predictive power. NISP is evaluated on several datasets with multiple CNN models and demonstrated to achieve significant acceleration and compression with negligible accuracy loss.

==> RIP_backup.tex <==
\section{Our Approach}
We follow a straightforward strategy to reduce Convolutional Neural Networks: pruning kernels of convolution layers and neurons in fully connected layers.
Trivial methods like random pruning or changing the number of neurons and kernels arbitrarily may result in huge degradation of the predictive power. We study the importance levels of neurons based on feature ranking of the final output, and then compute importance scores of intermediate neurons by measuring their effect on the final response.
Based on our study, we derive the Neuron Importance Score Propagation algorithm to efficiently propagate final response importance throughout the whole network.

%A naive way would be measuring the importance of neurons/kernels and prune them independently on a layer-by-layer basis, followed by iteratively retraining to compensate the loss of accuracy. However, since the feature dimension is very high and the datasets are usually in large scale, this method becomes computationally intractable. 


The framework overview is illustrated in Fig.~\ref{fig:spe}. Given a trained CNN, we first apply a feature ranking algorithm on this final response layer and obtain the importance score of each output neuron. Then, the Neuron Importance Sore Propagation (NISP) algorithm propagates importance scores throughout the network. 
% The theory and algorithm of RIP is described in Sec.~\ref{sec:rip}. 
Finally, the network is pruned based on the importance scores of neurons and fine-tuned to recover accuracy loss.
% The three components are described separately as follows.


%%%%%%%%%%%%%%%%% feature ranking
\subsection{Feature Ranking on the Final Response Layer}\label{sec:featrank}
The predictive capability of a neural network is highly dependent on the quality of the features in the final layer response. 
Existing work has demonstrated that a subset of important features, selected based on feature ranking of the network final response, still retains good predictive power \cite{Roffo_2015_ICCV}.
The intuition is that the final responses should play key roles in full network pruning since they are determined by intermediate neurons of a network. So, in the first step, we apply feature ranking on the final responses.

There are three major categories of feature selection: \emph{wrappers}, which score a subset of features using classifiers; 
\emph{embedding methods}, which implicitly select the features in the learning process of the classifier by regularization methods;
and \emph{filtering methods}, which exploit intrinsic properties of data, regardless of the classifiers \cite{nips2003,Roffo_2015_ICCV}.
Our method can be used with any feature selection model that can score individual features in a set with respect to classification power. We employ the recently introduced filtering method Inf-FS ~\cite{Roffo_2015_ICCV} because of its efficiency and effectiveness on CNN feature selection. Inf-FS first constructs an affinity graph whose nodes are the features to be scored and whose edges represent feature relations like correlation. A selection of features is represented by a path through the graph passing through those features. 
The model in Roffo \etal \shortcite{Roffo_2015_ICCV} utilizes properties of the power series of matrices to efficiently compute the  importance of a feature with respect to all the other features, \ie, it is able to integrate the importance of a feature over all paths in the affinity graph\footnote{Details of the method are provided in \cite{Roffo_2015_ICCV} and code for the method was taken from {\scriptsize\url{https://www.mathworks.com/matlabcentral/fileexchange/54763-infinite-feature-selection-2016}}.}. 



%%%%%%%%%%%%%%%%%%%%%%%%% RIP
\subsection{Neuron Importance Score Propagation (NISP)}\label{sec:rip}
Our goal is to decide which intermediate neurons to delete, given the importance scores of final responses, so that the predictive power of the network is maximally retained. We formulate this problem as a binary integer programming (optimization) and provide a  closed-form solution. Based on the theoretical analysis, we develop the Neuron Importance Score Propagation algorithm to efficiently compute the neuron importance for the whole network.


%\begin{figure}[h]
%\centering     
%\subfigure[]{\label{fig:proof1}\includegraphics[width=30mm]{image/proof1}}
%\subfigure[]{\label{fig:proof2}\includegraphics[width=30mm]{image/proof2}}
% \caption{Comparisons with layer-by-layer and magnitude based pruning baselines.}
%\caption{(a) is the case of two consecutive layers. (b) is the case that one low-level layer influences two high-level layers. $\beta$ and $\gamma$ are the importance of the high-level layers, and $\alpha$ is an indicator that determines whether a neuron is pruned in the low-level layer. $\mathbf{W}$ and $\mathbf{W'}$ are the weights between two layers. $\sigma$ is the activation function between layers.}
%\label{fig}
%Pruning based on magnitude
%\end{figure}

%To be general, any two layers of a CNN can be represented as Figure \ref{fig:proof1}, where 

\subsubsection{Problem Definition.}\label{sec:probdef}
Our goal is to delete neurons, keeping a fixed number of neurons and minimizing accuracy loss. While model accuracy is dependent on the feature importance of the final output, we define our objective as minimizing the weighted distance between the original final response and the final response after neurons are pruned in a specific layer. 
% We start with a definition of the general layer formulation. 
Throughout the rest of the paper, we use bold symbols to represent vectors and matrices. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% definition
\iffalse
Let $\mb x$ be the input to a layer. A layer can be represented using the following general form,
\begin{equation}
\label{proof1_objective_2}
f(\mb x)=\sigma(\mb w\mb x+\mathbf b)
\end{equation}
where $\sigma$ is an activation function, $\mb w,\mb b$ are weight and bias. The $j$-th output element of function $f$ is
$f_j(\mb x) = \sigma\left(\sum_{i} w_{i,j}x_i+b_j\right)$
where $x_i$ is the $i$-th element of $\mb x$.
\fi
%\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Most neural networks can be represented as a nested function. Thus, we define a network with depth $n$ as a function $F^{(n)}=f^{(n)}\circ f^{(n-1)}\circ\dots\circ f^{(1)}$. The $l$-th layer $f^{(l)}$ is represented using the following general form,
\begin{equation}
\label{proof1_objective_2}
f^{(l)}(\mb x)=\sigma^{(l)}(\mb w^{(l)}\mb x+\mathbf b^{(l)}),
\end{equation}
where $\sigma^{(l)}$ is an activation function and $\mb w^{(l)},\mb b^{(l)}$ are weight and bias. 
Networks with branch connections such as the skip connection in ResNet can be transformed to this representation by merging and expanding layers with added binary (zero or one) weights.

%The $j$-th output element of function $f^{(k)}$ is $f_j(\mb x) = \sigma\left(\sum_{i} w_{i,j}x_i+b_j\right)$ where $x_i$ is the $i$-th element of $\mb x$.

% \begin{definition}[Neuron prune indicator]\label{def:indicator}
We define the \textit{neuron importance score} as a non-negative value w.r.t. a neuron in the network, and use $\mb s_l$ to represent the vector of neuron importance scores  in the $l$-th layer. Suppose $N_l$ neurons are to be kept in the $l$-th layer after pruning; we define the \textit{neuron prune indicator} of the $l$-th layer to be a binary vector $\mb s^*_l$ which is computed based on the neuron importance scores $\mb s_l$ such that $s^*_{l,i}=1$ if and only if $s_{l,i}$ is among the highest $N_l$ values in $\mb s_l$. 

%This definition implies that given all neuron prune indicators $\{\mb s^*_1,\mb s^*_2,\ldots,\mb s^*_{N}\}$ where $\mb s^*_k$ is the indicator for keeping $k$ neurons after pruning, any non-negative vector $\mb s$ fulfilling such condition that $s_{i}\le s_{j}\Rightarrow s^*_{n,i}\le s^*_{n,j},\forall i,j,n$ is a feasible neuron importance score vector.
% \end{definition}

% \begin{proposition}[Neuron importance score]

% \begin{proof}
% Implied from Definition~\ref{def:indicator}.
% \end{proof}
% \end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% objective function
\subsubsection{Objective Function.}  Let $F^{(n)}$ be a neural network with $n$ layers. Suppose we have a dataset of $M$ samples, and each is represented using $\mb x^{(m)}_0$. For the $m$-th sample, we use $\mb x^{(m)}_l$ to represent the response of the $l$-th layer (which is the input to the $(l+1)$-th layer). So the final output of the network is $x^{(m)}_n$ and its corresponding neuron importance is $\mb s_n$. We define \begin{align}\label{eq:gnet}
G^{(i,j)}=f^{(j)}\circ f^{(j-1)}\circ\cdots\circ f^{(i)}
\end{align} as a sub-network of $F^{(n)}$ starting from the $i$-th layer to the $j$-th layer. Our goal is to compute for the $l$-th layer the neuron prune indicator $\mb s^*_l$ so that the influence of pruning the $l$-th layer on the important neurons of the final response is minimized. To accomplish this, we define an optimization objective w.r.t. the $l$-th layer neuron prune indicator, i.e.,
\begin{equation}
\label{proof1_objective}
\arg\min_{\mb s^*_l}\ \sum_{m=1}^M \mathcal{F}(\mb s^*_l|\mb x^{(m)}_l,\mb s_n; G^{(l+1,n)})~,
\end{equation}
which is accumulated over all samples in the dataset. The objective function for a single sample is defined as
\begin{equation}\label{proof1_objective2}
\mathcal{F}(\mb s^*_l|\mb x,\mb s_n; F)=\left\langle\ \mb s_n,\ |F(\mb x)-F(\mb s^*_l \odot \mb x)|\ \right\rangle,
\end{equation}
where $\langle\cdot,\cdot\rangle$ is dot product, $\odot$ is element-wise product and $|\cdot|$ is element-wise absolute value. The motivation behind Eq.~\ref{proof1_objective2} is that the difference between the responses produced by the original network and the one produced by the pruned network should be minimized w.r.t. important neurons.

%Eq.~\ref{proof1_objective2} can be re-written as
%\begin{align}\label{proof1_FSx}
%\mathcal{F}(\mb s^*_l|\mb x,\mb s_n; F)=\sum_j s_{nj}|F_j(\mb x) - F_j(\mb s^*_l\odot \mb x)|
%\end{align}
%where $s_{nj}$ is the $j$-th element of $\mb s_n$ and $F_j$ is the $j$-th output element of function $F$.

\subsubsection{Solution.}
The network pruning problem can be formulated as a binary integer program, finding the optimal neuron prune indicator in Eq.~\ref{proof1_objective}. However, it is hard to obtain efficient analytical solutions by directly optimizing Eq.~\ref{proof1_objective}. So we derive an upper bound on this objective, and show that a sub-optimal solution to the prune indicator can be obtained by minimizing the upper bound. More importantly, we find a feasible and efficient formulation for the importance scores of all neurons based on this sub-optimal solution. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Lemma 1
% \begin{lemma}\label{lemma}
% For any function $\sigma(\cdot)$ whose derivatives are bounded, there exists a positive constant $C$ such that 
% % $|\sigma(x)-]sigma(y)|\leqslant |x-y|$.
% \[|\sigma(x)-\sigma(y)|\le C|x-y|,\quad\forall x,y.\]
% \begin{proof} See appendix. \end{proof}
% \end{lemma}
% %%%%%%%%%%%%%%%%%%%%%%%

% %
% %Based on the Mean Value Theorem, 
% %\[\frac{\sigma(x)-\sigma(y)}{x-y} \leqslant \frac{d\sigma}{dx}\]
% %If $\frac{d\sigma}{dx} \leqslant C$, we have 
% %\[\frac{\sigma(x)-\sigma(y)}{x-y} \leqslant C, \text{suppose } y\leqslant x.\]
% %Then we have $|\sigma(x)-\sigma(y)|\leqslant C|x-y|$.
% %
% It is observed that most of the activation functions that are commonly used in neural networks have bounded derivatives such as Identity, ReLU, sigmoid, tanh, PReLu, \etc. When $\sigma(\cdot)$ is ReLu, $C=1$ is feasible for Lemma \ref{lemma}.


%For any function $\sigma(\cdot)$ that is Lipschitz-continuous, there exists a positive constant $C$ such that $|\sigma(x)-\sigma(y)|\le C|x-y|,\quad\forall x,y.$.
%When $\sigma(\cdot)$ is ReLU, $C=1$ is feasible for the above inequality.
%Thus, according to Lemma \ref{lemma}, we have
%\begin{align}
%\label{proof1_fx}
%\textstyle|f_j&(\mb x)-f_j(\mb s_x \odot \mb x)|\nonumber\\
%&\textstyle=\left|\sigma(\sum_i w_{i,j}x_i+b_j)-\sigma(\sum_i w_{i,j} x_is_{xi}+b_j)\right| \nonumber \\
%&\textstyle\le C_\sigma\left|\sum_i w_{i,j}x_i(1-s_{xi})\right|\nonumber\\
%&\textstyle \le C_\sigma \sum_i |w_{i,j}||x_i|(1-s_{xi}).
%\end{align}
%Substituting Eq.~\ref{proof1_fx} into Eq.~\ref{proof1_FSx}, we have
%\begin{align}
%\mathcal{F}(\mb s_x|\mb x)&\le \sum_js_{yj}C_\sigma\sum_i|w_{i,j}||x_i|(1-s_{xi})\nonumber\\
%&=C_\sigma\sum_i |x_i|(1-s_{xi})\sum_j s_{yj}|w_{i,j}|~.
%\end{align}
%Let $r_{xi}=\sum_j s_{yj}|w_{i,j}|$, we have
%\begin{align}
%\sum_{k=1}^N \mathcal{F}(\mb s_x|\mb x^{(k)}))&\le \sum_{k=1}^NC_\sigma\sum_i |x_i^{(k)}|(1-s_{xi})r_{xi}\nonumber\\
%&=C_\sigma\sum_i(1-s_{xi})r_{xi}\sum_{k=1}^N|x_i^{(k)}|
%\end{align}
%where $N$ is the total number of samples. In practice, $N$ is a large value, so we can approximate $\sum_{k=1}^N|x_i^{(k)}|=N\mathop{\mathbb{E}}[|x_i|]$. Then there must exists a constant value $C_x$ such that $C_x\ge \mathop{\mathbb{E}}[|x_i|], \forall i$. Therefore,
%\begin{align}
%\sum_{k=1}^N \mathcal{F}(\mb S_x|\mb X^{(k)}))\le C_\sigma C_x\sum_i(1-s_{xi})r_{xi}
%\end{align}
%which reveals the upper bound of the objective in Eq.~\ref{proof1_objective}. So we optimize our objective by minimizing its upper-bound. 

%Based on the assumption that $x_i$ is i.i.d., which usually holds for normalized data such as image mean substraction and batch normalization (BN) \cite{BN}, then there exists a $\mu$ such that $E[\ |x_i|\ ] = \mu,\, \forall i$. Summing up the upper bound over all $N$ samples, 


%Then, we derive the upper-bound of the objective function as:
%\begin{equation}
%\begin{aligned}
%\label{proof1_upperbound}
%U(F) &\leqslant \sum_j \beta_j\sum_i C(1-\alpha_i) |w_{i,j}||X_i| %\\\nonumber
%&= \sum_i C |X_i| (1-\alpha_i) \sum_j \beta_j|w_{i,j}|.
%\end{aligned}
%\end{equation}
%
%We assume $X_i$ is drawn i.i.d from a distribution $D$, which usually holds for the input layer due to image mean subtraction and in middle layers due to Batch Normalization (BN)\cite{BN}. By summing the $U(F)$ for all responses, we have 
%\begin{align}
%\label{proof1_upperfbound2}
%\sum_{k=1}^N \mathcal{F}_{ub}(\mb S_x|\mb X^{(k)}))&\propto \sum_k\sum_i |x_i^{(k)}|(1-s_{xi})r_i\nonumber\\
%&\propto \sum_i \left(\sum_{k=1}^N|x_i^{(k)}|\right)(1-s_{xi})r_i\nonumber\\
%&= \sum_i N\mu(1-s_{xi})r_i\nonumber\\
%&\propto\sum_i(1-s_{xi})r_i
%\end{align}
%where $\mu$ is the expectation of $|x_i|$.

% %%%%%%%%%%%%%%%%%%%%%% Lemma 2
% \begin{lemma}\label{lemma2}
% Suppose a layer is defined as $f(\mb x)=\sigma(\mb w\mb x+\mb b)$ where the activation derivative $\sigma'$ is bounded, then for any $\mb x, \mb y$, there exists a constant $C_\sigma$ such that
% \begin{align}
% |f_j(\mb x)-f_j(\mb y)|\le C_\sigma\sum_i |w_{i,j}|\cdot|x_i-y_i|~.\nonumber
% \end{align}
% \begin{proof}
% Based on Lemma \ref{lemma}. See appendix.
% \end{proof}
% \end{lemma}
Recall that the $k$-th layer is defined as $f^{(k)}(\mb x)=\sigma^{(k)}(\mb w^{(k)}\mb x+\mb b^{(k)})$. We assume the activation function $\sigma^{(k)}$ is Lipschitz continuous since it is generally true for most of the commonly used activations in neural networks  such as Identity, ReLU, sigmoid, tanh, PReLU, etc. Then we know for any $\mb x,\mb y$, there exists a constant $C_\sigma^{(k)}$ such that
\begin{align}
    |\sigma^{(k)}(\mb x)-\sigma^{(k)}(\mb y)|\le C_\sigma^{(k)}|\mb x-\mb y|~.
\end{align}
Then it is easy to see that
\begin{align}\label{lemma2}
|f^{(k)}(\mb x)-f^{(k)}(\mb y)|\le C_\sigma^{(k)}|\mb w^{(k)}|\cdot|\mb x-\mb y|~.
\end{align}
where $|\cdot|$ is the element-wise absolute value. From Eq.~\ref{eq:gnet}, we see that $G^{(i,j)}=f^{(j)}\circ G^{(i,j-1)}$. Therefore, we have,
\begin{align}
    &|G^{(i,j)}(\mb x)-G^{(i,j)}(\mb y)|\nonumber\\
    &~~~~~~~\le C_\sigma^{(j)}|\mb w^{(j)}||G^{(i,j-1)}(\mb x)-G^{(i,j-1)}(\mb y)|~.\label{eq:G}
\end{align}
By applying Eq.~\ref{lemma2} and repeatedly applying Eq.~\ref{eq:G} for $j=i, i+1\ldots, n$, we have
\begin{align}
   & |G^{(i,n)}(\mb x)-G^{(i,n)}(\mb y)|\le C_\Sigma^{(i,j)}\mb W^{(i,j)}|\mb x-\mb y|,\label{eq:intermediate}
\end{align}
where $\mb W^{(i,j)}=|\mb w^{(j)}||\mb w^{(j-1)}|\cdots|\mb w^{(i)}|$ and $C_\Sigma^{(i,j)}=\prod_{k=i}^j C_\sigma^{(k)}$.
Substituting $\mb x = \mb x_l^{(m)},\mb y=\mb s^*_l\odot\mb x_l^{(m)},i=l+1$ into Eq.~\ref{eq:intermediate}, we have
\begin{align}
&|G^{(l+1,n)}(\mb x^{(m)}_l)-G^{(l+1,n)}(\mb s^*_l\odot\mb x^{(m)}_l)|\nonumber\\
&~~~~~~\le C_\Sigma^{(l+1,n)}\mb W^{(l+1,n)}|\mb x^{(m)}_l-\mb s^*_l\odot\mb x^{(m)}_l|~.
\end{align}
Since $\mb s_n$ is a non-negative vector,
\begin{align}
&\mathcal{F}(\mb s^*_l|\mb x^{(m)}_l,\mb s_n; G^{(l+1,n)})\nonumber\\
&~~~~=\langle\mb s_n, |G^{(l+1,n)}(\mb x^{(m)}_l)-G^{(l+1,n)}(\mb s^*_l\odot\mb x^{(m)}_l)|\rangle\\
&~~~~\le \langle\mb s_n, C_\Sigma^{(l+1,n)}\mb W^{(l+1,n)}|\mb x^{(m)}_l-\mb s^*_l\odot\mb x^{(m)}_l|\rangle\\
&~~~~=C_\Sigma^{(l+1,n)}\langle{\mb W^{(l+1,n)}}^\intercal\mb s_n, (\mb 1-\mb s^*_l)\odot\mb |x^{(m)}_l|\rangle~.
\end{align}
Let us define $\mb r_l={\mb W^{(l+1,n)}}^\intercal\mb s_n$; then
\begin{align}
&\sum_{m=1}^M \mathcal{F}(\mb s^*_l|\mb x^{(m)}_l,\mb s_n; G^{(l+1,n)})\nonumber\\
&~~~~~~\le C_\Sigma^{(l+1,n)}\sum_{m=1}^M \langle\mb r_l,(\mb 1-\mb s^*_l)\odot|\mb x^{(m)}_l|\rangle\\
&~~~~~~=C_\Sigma^{(l+1,n)}\sum_{m=1}^M \sum_i r_{l,i}(1-s^*_{l,i})|x^{(m)}_{l,i}|\\
&~~~~~~=C_\Sigma^{(l+1,n)}\sum_ir_{l,i}(1-s^*_{l,i})\sum_{m=1}^M|x^{(m)}_{l,i}|~.
\end{align}
Since $|\mb x^{(m)}_{l,i}|$ is bounded, there must exist a constant $C_x$ such that $\sum_{m=1}^M |x^{(m)}_{l,i}|\le C_x,\forall i$. Thus, we have
\begin{align}
&\sum_{m=1}^M \mathcal{F}(\mb s^*_l|\mb x^{(m)}_l,\mb s_n; F^{(l+1)})\le C\sum_ir_{l,i}(1-s^*_{l,i}),\label{eq:upbound}
\end{align}
where $C=C_\Sigma^{(l+1,n)}C_x$ is a constant factor.


%%%%%%%%%%%%%%%%%%%%%%%%% comment begin
\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%% theorem
\begin{proposition}\label{theorem}
Let $F^{(n)}=f^{(n)}\circ f^{(n-1)}\circ\dots\circ f^{(1)}$ be a neural network with depth $n$ where the $l$-th layer is defined as $f^{(l)}(\mb x)=\sigma^{(l)}(\mb w^{(l)}\mb x+\mb b^{(l)})$ and $\sigma^{(l)}$ is Lipschitz continuous. Then there exists a constant value $C$ such that
\begin{align}\label{eq:layer}
    \sum_{m=1}^M\mathcal{F}(\mb s^*_l|\mb x^{(m)}_l, \mb s_n; F^{(l+1)})\le C\langle\ \mb 1-\mb s^*_l,\ \mb W^\intercal\mb s_n\ \rangle
    % \label{eq:upbound}
\end{align}
where $M$ is the total number of samples and large, $\langle\cdot,\cdot\rangle$ is the dot product, and $\mb W=|\mb w^{(n)}||\mb w^{(n-1)}|\cdots|\mb w^{(l+1)}|$.
\begin{proof}Let $F^{(k)}=f^{(k)}\circ f^{(k-1)}\circ\dots\circ f^{(1)}$ be a sub-network of $F^{(n)}$ and $F^{(0)}(\mb x)=\mb x$ is the identity. Let us define
\begin{align}
G^{(k)}_j=|F_{j}^{(k)}(\mb x)-F_{j}^{(k)}(\mb s^*_x\odot\mb x)|~,\nonumber
\end{align}
then, for any $n\ge 1$, we have
\begin{align}
    G^{(k)}_j=|f^{(k)}_j(F^{(k-1)}(\mb x^{(m)}_l))-f^{(k)}_j(F^{(k-1)}(\mb s^*_l\odot\mb x^{(m)}_l))|\nonumber~.
    \end{align}
    According to Eq.~\ref{eq:layer}, there exists $C_\sigma^{(k)}$ such that
    \begin{align}
    G^{(k)}_j
    &\le C_\sigma^{(k)}\sum_{i}|w_{i,j}^{(k)}|\cdot|F^{(k-1)}_{i}(\mb x)-F_{i}^{(k-1)}(\mb s^*_x\odot\mb x)|\nonumber\\
    &= C_\sigma^{(k)}\sum_{i}|w_{i,j}^{(k)}|G^{(k-1)}_i\nonumber
\end{align}
whose matrix form is
$\mb G^{(k)}\le C_\sigma^{(k)}|\mb w^{(k)}|\mb G^{(k-1)}$.
By applying the same inequalities for $k=1,2,\ldots,n$, we have
\begin{align}
\mb G^{(n)}\le C_\Sigma\mb W\mb G^{(0)},\nonumber
\end{align}
where $C_\Sigma=\prod_{k=1}^n C_\sigma^{(k)}$, $\mb W=|\mb w^{(n)}||\mb w^{(n-1)}|\cdots|\mb w^{(1)}|$, and $\mb G^{(0)}=|\mb x - \mb s^*_x\odot\mb x|$. Then we have,
\begin{align}
\mathcal{F}(\mb s^*_x|\mb x, \mb s_y; F^{(n)})&=\sum_j s_{yj}G_j^{(n)}\nonumber\\
&\le \sum_j s_{yj}C_\Sigma\sum_iW_{i,j}|x_i - s^*_{xi}x_i|\nonumber\\
&= C_\Sigma\sum_i |x_i|(1-s^*_{xi})\sum_j W_{i,j}s_{yj}\nonumber~.
\end{align}
Let $\mb r=\mb W^\intercal \mb s_y$ (i.e., $r_i=\sum_j W_{i,j}s_{yj}$), then we have
\begin{align}
\sum_{m=1}^M\mathcal{F}(\mb s^*_x|\mb x^{(m)}, \mb s_y; F^{(n)})&\le C_\Sigma\sum_{m=1}^M\sum_i |x_i^{(m)}|(1-s^*_{xi})r_{i}\nonumber\\
&=C_\Sigma\sum_i(1-s^*_{xi})r_i\sum_{m=1}^M|x_i^{(m)}|\nonumber~.
\end{align}
Since the total number $M$ of input samples is a large value, hence we can approximate  $\sum_{m=1}^M|x_i^{(m)}|=M\mathop{\mathbb{E}}[|x_i|]$,  according to the law of large numbers. Then, there must exists a constant value $C_x$ such that $C_x\ge \mathop{\mathbb{E}}[|x_i|], \forall i$. Thereafter,
\begin{align}
\sum_{m=1}^M\mathcal{F}(\mb s^*_x|\mb x^{(m)}, \mb s_y; F^{(n)})\le C_\Sigma C_x\sum_i(1-s^*_{xi})r_i~.\label{eq:theo-last}
\end{align}
Let $C=C_\Sigma C_x$ and we see Eq.~\ref{eq:theo-last} is equivalent to Eq.~\ref{eq:upbound}.
%\begin{align}\pushQED{\qed} 
%\sum_{m=1}^M\mathcal{F}(\mb s^*_x|\mb x^{(m)}, \mb s_y; F^{(n)})\le C\langle\ \mb 1-\mb s^*_x,\ \mb W^\intercal\mb s_y\ \rangle~.~~~~~~~~~~~~\qedhere\nonumber
%\end{align}
\end{proof}
\end{proposition}

\fi
%%%%%%%%%%%%%%%%%%%%%%% comment end

Eq.~\ref{eq:upbound} reveals an upper-bound of our objective in Eq.~\ref{proof1_objective}. Thus, we minimize this upper-bound, i.e.,
\begin{align}
\arg\min_{\mb s^*_l}\sum_ir_{l,i}(1-s^*_{l,i})\Leftrightarrow\arg\max_{\mb s^*_l}\ \sum_is^*_{l,i}r_{l,i}~.\label{suboptimal}
\end{align}
%So it is equivalent to
%\begin{align}\label{theory:finalobjective}
%\arg\max_{\mb s^*_x}\ \sum_is^*_{xi}r_i~.
%\end{align}
The optimal solution to Eq.\ref{suboptimal} is sub-optimal with respect to the original objective in Eq.~\ref{proof1_objective}, however it still captures the importance of neurons. It is easy to see that if we keep $N_x$ neurons in the $l$-th layer after pruning, then the solution to Eq.~\ref{suboptimal} is that $s^*_{l,i}=1$ if and only if $r_{l,i}$ is among the highest $N_x$ values in $\mb r_l$. According to the definition of neuron prune indicator in Sec.~\ref{sec:probdef}, $\mb r_l={\mb W^{(l+1,n)}}^\intercal\mb s_n$ is a feasible solution to the importance scores of the $l$-th layer response. This conclusion can be applied to every layer in the network. Based on this result, we define the neuron importance of a network as follows.
 %We can see, for any $N_x$, $r_i\le r_j\Rightarrow s^*_{xi}\le x^*_{xj}$. 

\begin{definition}[Neuron importance score]\label{def:ri}
Given a neural network $F^{(n)}$ containing $n$ layers and the importance score  $\mb s^{(n)}$ of the last layer response, the importance score of the $k$-th layer response can be computed as 
\begin{align}
\mb s_k=|\mb w^{(k+1)}|^\intercal|\mb w^{(k+2)}|^\intercal\cdots|\mb w^{(n)}|^\intercal \mb s_n,
\end{align}
where $\mb w^{(i)}$ is the weight matrix of the $i$-th layer.
\end{definition}

An important property of neuron importance is that it can be computed recursively (or propagated) along the network.
\begin{proposition}[Neuron importance score propagation] \label{def:rip} The importance score of the $k^\text{th}$ layer response can be propagated from the importance score of the $(k+1)^\text{th}$ layer by
\begin{align}
\mb s_k=|\mb w^{(k+1)}|^\intercal\mb s_{k+1},\label{eq:rip}
\end{align}
where $\mb w^{(k+1)}$ is the weight matrix of the $(k+1)^\text{th}$ layer.
\end{proposition}

%Corollary \ref{corollary:rip} reveals that the importance of neurons in a low-level layer activation can be propagated from its direct higher-level layer activation by the magnitude of weights of the layer in between.

\subsubsection{Algorithm}
We propose the \textit{Neuron Importance Score Propagation} (NISP) algorithm based on Proposition~\ref{def:rip}. Initially, we have the importance score of every neuron in the final layer of the network. Definition~\ref{def:ri} shows that the importance score of every other layer in the network is directly correlated with the importance of the final response. However, instead of computing the importance expensively using Definition~\ref{def:ri}, we see from Eq.~\ref {eq:rip} that the importance score of a lower layer can be propagated directly from the adjacent layer above it. An equivalent form of Eq.~\ref{eq:rip} is
\begin{equation}
    \textstyle s_{k,j}=\sum_i |w^{(k+1)}_{i,j}|s_{k+1,i},\label{eq:prop}
\end{equation}
where $s_{k,j}$ is the importance score of the $j$-th neuron in the $k$-th layer response. 

We conclude from Eq.~\ref{eq:prop} that the importance of a neuron is a weighted sum of all the subsequent neurons that are directly connected to it. This conclusion also applies to the case when the network has branch connections, i.e., a layer is directly connected with multiple layers.
% \footnote{\label{supp}See supplementary material for more details.}. 
The importance of batch normalization layers is propagated identically since the connections between neurons form a one-one mapping. An exception is the max-pooling layer in which we assume a uniform probability for each neuron to be the maximum in the window. So in our implementation, the NISP of max-pooling is treated in the same way as average-pooling. Our algorithm starts with the final layer importance and repeats the propagation (Eq.~\ref{eq:prop}) to obtain the importance of all neurons in the network with a single backward pass (Fig.~\ref{fig:spe}).
% \footref{supp}. 

%RIP efficiently measures the importance of neurons and kernels of an entire deep neural network consistently as shown in Figure \ref{fig:spe}. Importantly, it is able to assign credit to neurons that have important contributions to future layers but which might otherwise be scored as unimportant if evaluated as an independent feature.

%The importance of a neuron in a low-level layer is computed based on the importance of its next layer's neurons and the weights between them as follows:
%\begin{equation}
%\label{RIP}
%s^{(k)}_j=\sum_i s^{(k+1)}_j |w^{(k)}_{i,j}|
%\end{equation}
%where $n_i$ is the $i^{th}$ neuron in the %low-level layer, $\beta_j$ is the importance of %the $j^{th}$ neuron in the next layer and %$w_{i,j}$ is the weight between them. We propagate %the importance from the final response layer to %the lowest layer of a CNN layer-by-layer using %Eq.~\ref{RIP}.

\subsection{Pruning Networks Using NISP} \label{sec:prune} Given target pruning ratios for each layer, we propagate the importance scores, compute the prune indicator of neurons based on their importance scores 
% (Definition~\ref{def:indicator}) 
and remove neurons with prune indicator value $0$. The importance propagation and layer pruning happens jointly in a single backward pass, and the importance of a pruned neuron is not propagated to any further low-level layers. For most of the layers, e.g., fully connected layers, we prune the neurons independently. For a convolution layer, we prune a whole channel of neurons at the same time. Suppose a convolution layer has an output tensor with $C$ channels, then the assignment of prune indicator is essentially optimizing the same objective function in Eq.~\ref{suboptimal} but with an additional constraint that a set of neurons within the same channel should have the same prune indicator value. In this case, Eq.~\ref{suboptimal} becomes $\arg\max \sum_{i=c}^C s_{l,c}^\text{chan*}\left( \sum_{j\in idx_{l,c}^\text{chan}}r_{l,j}\right)$ where $s_{l,c}^\text{chan*}$ is the prune indicator of the $c$-th channel of the $l$-th layer and $idx_{l,c}^\text{chan}$ is the set of indices of neurons in the $c$-th channel of the $l$-th layer. Thus, the importance score of a channel can be computed as the summation of the importance scores of neurons within this channel\footnote{More details can be found in supplementary materials.}.
%using equation \eqref{kernelRIP}:
%\begin{equation}
%\label{kernelRIP}
%RI_{c}=\sum_{i,j} RI_{i,j,c},
%\end{equation}


% Given the importance score of a neuron, we first identify the positions in the previous layer that are used as its input, then back propagate the importance to the positions proportional to the weights. 
% We only back propagate the importance scores of the selected feature extractors to the previous layers and ignore the pruned ones.
% The RIP process can be divided into three classes: from a 1-way tensor to a 1-way tensor, e.g. between FC layers; from a 1-way tensor to a 3-way tensor, e.g., from an FC layer to a conv/pooling layer; from a 3-way tensor to a 3-way tensor, e.g., from a pooling layer to a conv layer.
% There are some other layers such as non-linearity layer (e.g. ReLU) and regularization layer (e.g. Dropout), and the RIP process on those layers can be simplified due to their properties. 
% We simplify the RIP method by ignoring the back propagation of bias.
% because there is no connection between cross-channel biases, and the importance.

% \subsection{RIP: from 1-way tensor to 1-way tensor}

% Given an FC layer with $M$ input neurons and $N$ output neurons, the $N
% \text{-}by\text{-}1$ importance score vector ($\mathbf{IS}$) of the output feature is $\mathbf{IS_{FC_{out}}}=\left [{IS_{FC_{out}}}_1,{IS_{FC_{out}}}_2 \dots {IS_{FC_{out}}}_N\right ]^\text{T}$. 
% We use $\mathbf{W_{FC}}\in \mathbb{R}^{M\times N}$ to denote the weights of the FC layer. The importance score vector of the input neurons is:

% \begin{equation}
% \label{IS_FC_FC}
% \mathbf{IS_{FC_{in}}}=\mathbf{W_{FC}}  \cdot  \mathbf{IS_{FC_{out}}}.
% \end{equation}

% \subsection{RIP: from 1-way tensor to 3-way tensor}
% Given an FC layer with a 3-way tensor as input and $N$ output neurons, the input has a size of $X \times X \times C$, where $X$ is the spatial size and $C$ is the number of input channels. The input can be the response of a convolutional layer or a pooling layer.
% We use $\mathbf{W_{FC}}\in \mathbb{R}^{(X^2 \times C)\times N}$ to denote the weights of the FC layer. The flattened importance score vector $\mathbf{IS_{in}} \in \mathbb{R}^ {(X^2 \times C)\times 1}$ of the input tensor is:
% \begin{equation}
% \label{IS_FC_conv}
% \mathbf{IS_{in}}=\mathbf{W_{FC}} \cdot \mathbf{IS_{FC_{out}}}.
% \end{equation}

% \subsection{RIP: from 3-way tensor to 3-way tensor}
% % The RIP from a 3-way tensor to a 3-way tensor is much more complicated than the first two cases because of the large number of forward propagation operations between the input and output responses.
% We derive the RIP method for a convolutional layer, which is the most complicated case of RIP between 3-way tensors.
% The RIP method for pooling and local response normalization (LRN) can be derived similarly.
% We describe them in the supplementary materials.

% For a convolutional layer with the input 3-way tensor $\mathbf{{conv_{in}}} \in \mathbb{R}^ {X\times X \times N }$ and output tensor $\mathbf{{conv_{out}}} \in \mathbb{R}^ {Y\times Y \times F )}$, the filter size is $k$, stride is $s$ and the number of padded pixels is $p$.
% During the forward propagation, convolution consists of multiple inner products between a kernel $\mathbf{k}_f \in \mathbb{R}^ {k\times k \times N}$, and multiple corresponding receptive cubes to produce an output response.
% Fixing input channel $n$ and output channel $f$, the spatial convolutional kernel is $\mathbf{k}_{fn}$. For position $i$ in the $n^{th}$ channel of the input tensor, the corresponding response of the output channel $f$ at position $i$ is defined as \eqref{fw_conv}:
% \begin{equation}
% \label{fw_conv}
% R_f(i)=\sum_n \mathbf{k}_{fn} \cdot \mathbf{in}(i),
% \end{equation}
% where $\mathbf{in}(i)$ is the corresponding 2-D receptive field. 
% Given the importance score cube of the output response $\mathbf{{IS_{out}}} \in \mathbb{R}^ {Y \times Y \times F}$, we use a similar linear computation to back propagate the importance score from the output response to the input:
% \begin{equation}
% \label{bw_conv}
% IS_n(i)=\sum_f \mathbf{k}_{fn} \cdot \mathbf{IS}_{out}(i),
% \end{equation}
% where $IS_n(i)$ is the importance score of position $i$ in the $n^{th}$ input channel, and $\mathbf{IS}_{out}(i)$ is the corresponding 2-D matrix that contains the output positions whose responses come from the value of that input position during forward propagation.
% We back propagate the importance proportionally to the weights as described in Algorithm \ref{convBP}.
% \begin{algorithm}
% \caption{RIP: convolutional layer}\label{convBP}
% \begin{algorithmic}[1]
% \State $\mathbf{Input: }  \text{ weights of the conv layer } \mathbf{W} \in \mathbb{R}^ {X\times X \times N \times F} $
% \State $\text{, flattened importance score of the $f^{th}$ output channel }$ \State $\mathbf{IS}_{out}^f \in \mathbb{R}^ {1 \times( X \times X )}$
% \For {n in 1 \dots N}
% \For {f in 1 \dots F}
% \State $\mathbf{k}_{fn}  \gets \mathbf{W}[:,:,n,f]$
% \State $\text{Construct } \mathbf{BP}_{conv}^{fn}$ as \eqref{BP_conv} and \eqref{b_c}
% \State $\mathbf{IS}_{in}^{fn} \gets \mathbf{IS}_{out}^f \cdot
% \mathbf{BP}_{conv}^{fn}$
% \EndFor
% \State $\mathbf{IS}_{in}^{n} \gets \sum_f \mathbf{IS}_{in}^{fn}$
% \EndFor
% \State $\mathbf{IS}_{in} \gets [\mathbf{IS}_{in}^{1},\mathbf{IS}_{in}^{2} \dots, \mathbf{IS}_{in}^{N}]$
% \State \text{end}
% \end{algorithmic}
% \end{algorithm}

% The back propagation matrices used in algorithm \ref{convBP} are defined in \eqref{BP_conv} and \eqref{b_c}
% \begin{equation}
% \label{BP_conv}
% \mathbf{BP}_{conv}^{fn}=\left[
% \begin{aligned}
% \mathbf{b}_1^{fn} \dots\ \  \mathbf{b}_j^{fn}  \ \ & \dots \,\mathbf{b}_k^{fn}  \\
% \mathbf{b}_1^{fn} \dots\ \  &\mathbf{b}_j^{fn}  \ \  \dots \,\mathbf{b}_k^{fn}  \\
% \vdots \\
% \mathbf{b}_1^{fn} &\dots\ \  \mathbf{b}_j^{fn}  \ \ & \dots \,\mathbf{b}_k^{fn}  \\
% \end{aligned}
% \right],
% \end{equation}
% where $\mathbf{b}_c^i$ is the building block of size $Y \times X$ defined as:
% \begin{equation}
% \label{b_c}
% \mathbf{b}_{i}^{fn}=\left[
% \begin{aligned}
% \mathbf{k}_{fn}[i,1] \dots\ \  & \dots \mathbf{k}_{fn}[i,k]   \\
% \mathbf{k}_{fn}[i,1]&\dots \ \  \dots \mathbf{k}_{fn}[i,k]  \\
% \vdots \\
% &\mathbf{k}_{fn}[i,1]  \dots\ \   \dots \mathbf{k}_{fn}[i,k] 
% \end{aligned}
% \right],
% \end{equation}

% Equation \eqref{bw_conv} implies that the back propagation of importance score between 3-way tensors in convolutional layers can be decomposed into back propagation between 2-D matrices. 
% Fixing the input channel $n$ and the output channel $f$, the input layer size is $X \times X$ and the output size is $Y \times Y$. 
% Given the flattened importance score vector $\mathbf{IS_{out}}^f \in \mathbb{R}^ {1\times (Y \times Y )}$ of the output layer, the back propagation matrix $\mathbf{BP}_{conv}^{fn} \in \mathbb{R}^ { (Y \times Y ) \times (X \times X)}$ is used to map from $\mathbf{IS_{out}}^f$ to the importance score of input layer $\mathbf{IS_{in}}^{fn} \in \mathbb{R}^ {1\times (X \times X )}$. 
% $\mathbf{BP}^{fn}_{conv}(i,j)\neq0$,  implies that the $i^{th}$ position in the output layer comes from a convolution operation with the $j^{th}$ position in the input layer, and we back propagate the importance score between the two positions.
% We use a $Y \times X$ matrix $\mathbf{b}^{fn}_i$ to represent the mapping between a row in the output layer to the corresponding row in the input layer.
% In each row of $\mathbf{b}^{fn}_i$, there are $k$ non-zeros since each position in the output layer is obtained from a region with width $k$ of the input layer. The non-zeros of each row of $\mathbf{b}^{fn}_i$ are the $i^{th}$ row of the convolutional kernel $\mathbf{k}_{fn}$.
% The offset of the beginning of the weights in each row is the stride $s$. 
% The entire back propagation matrix $\mathbf{BP}_{conv}^{fn}$ is a block matrix with each submatrix being a $Y \times X$ matrix of either $\mathbf{b}_i^{fn}$ or a zero matrix. 
% Each row of $\mathbf{BP}_{conv}^{fn}$ has $\mathbf{b}_1^{fn}$ to $\mathbf{b}_k^{fn}$ because the height of a convolutional kernel is $k$. 
% The offset of the beginning of the $\mathbf{b}$s in each row of $\mathbf{BP}_{conv}^{fn}$ is the stride s. 
% We use the case when $X=4, Y=2, k=3, s=1$ as an example shown in Figure \ref{fig:conv}.

% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=0.95\linewidth]{image/conv.pdf}
% \end{center}
%   \caption{Importance score back propagation: Convolutional layer. $X=4, Y=2, k=3, s=1$. Fixing the $f^{th}$ input channel and $c^{th}$ output channel, the upper-left X-by-X grid is the corresponding input feature map, and the upper-right Y-by-Y grid is the output map after convolution is applied. $\mathbf{k}_{fc}$ is the corresponding 2D convolutional kernel. Given the flattened importance score vector for the output feature map $\mathbf{IS_{out}}^{f,c}$, we use $\mathbf{BP}_{conv}$ to back propagate the importance and obtain $\mathbf{IS_{in}}^{f,c}$, which contains the importance scores of the input feature map. The structure of $\mathbf{BP}_{conv}$ is determined by the kernel size k and stride s. }
% \label{fig:conv}
% \end{figure}


% \subsection{Other Layers}
% The RIP is difficult to compute between the output response and the input for the ReLU layer and Dropout layers because the operations are nonlinear. For a ReLU layer, since the ReLU operation is only conducted in isolation on a position without crossing channels or involving any other positions, we assume the importance score can be back propagated through the ReLU layer unchanged. Similarly, we back propagate using the identity matrix for dropout layers because all neurons share the same dropout possibility.

